Performance portability through machine learning guided kernel selection in SYCL libraries

Automatically tuning parallel compute kernels allows libraries and frameworks to achieve performance on a wide range of hardware, however these techniques are typically focused on finding optimal kernel parameters for particular input sizes and parameters. General purpose compute libraries must be able to cater to all inputs and parameters provided by a user, and so these techniques are of limited use. Additionally, parallel programming frameworks such as SYCL require that the kernels be deployed in a binary format embedded within the library. As such it is impractical to deploy a large number of possible kernel configurations without inflating the library size. Machine learning methods can be used to mitigate against both of these problems and provide performance for general purpose routines with a limited number of kernel configurations. We show that unsupervised clustering methods can be used to select a subset of the possible kernels that should be deployed and that simple classification methods can be trained to select from these kernels at runtime to give good performance. As these techniques are fully automated, relying only on benchmark data, the tuning process for new hardware or problems does not require any developer effort or expertise.

==> Makefile <==

PACKAGE = parco-kernel-sel-2020
NAME = auto-kernel-sel
SECTIONS = \
					 introduction.tex \
					 matmul.tex \
					 pruning.tex \
					 classification.tex \
					 vgg.tex \
					 conclusions.tex \

IMAGES = \
				 images/amd_config_counts.pdf \
				 images/intelcpu_config_counts.pdf \
				 images/amd_pca_variance.pdf \
				 images/intelcpu_pca_variance.pdf \
				 images/amd_error_classes.pdf \
				 images/intelcpu_error_classes.pdf \
				 images/vgg_times.pdf \
				 images/amd_sample_flops.pdf \

all: ${NAME}.pdf

%.pdf: %.tex ${SECTIONS} ${IMAGES} ${TABLES} bibliography.bib
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	  do pdflatex $<; done

clean_pictures:
	$(RM) ${IMAGES}

data/amd.csv: data/results.tar.gz
	cd data; tar mxf results.tar.gz; cd ..

data/%.csv: data/amd.csv

images/amd_config_counts.pdf: scripts/plot_max_counts.py
	python3 scripts/plot_max_counts.py

images/intelcpu_config_counts.pdf: scripts/plot_max_counts.py
	python3 scripts/plot_max_counts.py

images/amd_sample_flops.pdf: scripts/plot_amd_sample.py data/amd.csv
	python3 scripts/plot_amd_sample.py

images/amd_pca_variance.pdf: scripts/plot_pca_variance.py data/amd.csv
	python3 scripts/plot_pca_variance.py

images/intelcpu_pca_variance.pdf: scripts/plot_pca_variance.py data/intelcpu.csv
	python3 scripts/plot_pca_variance.py

images/amd_error_classes.pdf: scripts/plot_error_classes.py data/amd_prune.csv
	python3 scripts/plot_error_classes.py

images/intelcpu_error_classes.pdf: scripts/plot_error_classes.py data/intelcpu_prune.csv
	python3 scripts/plot_error_classes.py

images/vgg_times.pdf: scripts/plot_vgg_times.py data/vgg.csv
	python3 scripts/plot_vgg_times.py

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.tar.gz

archive: all clean
	COPYFILE_DISABLE=1 \
		tar -C .. -acf ../$(PACKAGE).tar.gz \
		--exclude '*~' \
		--exclude '*.tar.gz' \
		--exclude '*.tgz' \
		--exclude '*.zip' \
		--exclude '.git*' \
		--exclude '$(PACKAGE)/data' \
		--exclude '$(PACKAGE)/scripts' \
		--exclude '$(NAME).pdf' \
		$(PACKAGE)
	mv ../$(PACKAGE).tar.gz .

